Object-Centric World Model for Language-Guided Manipulation

A world model is essential for an agent to predict the future and plan in domains such as autonomous driving and robotics. To achieve this, recent advancements have focused on video generation, which has gained significant attention due to the impressive success of diffusion models. However, these models require substantial computational resources. To address these challenges, we propose a world model leveraging object-centric representation space using slot attention, guided by language instructions. Our model perceives the current state as an object-centric representation and predicts future states in this representation space conditioned on natural language instructions. This approach results in a more compact and computationally efficient model compared to diffusion-based generative alternatives. Furthermore, it flexibly predicts future states based on language instructions, and offers a significant advantage in manipulation tasks where object recognition is crucial. In this paper, we demonstrate that our latent predictive world model surpasses generative world models in visuo-linguo-motor control tasks, achieving superior sample and computation efficiency. We also investigate the generalization performance of the proposed method and explore various strategies for predicting actions using object-centric representations.

==> table/ablation.tex <==
\captionsetup[table]{skip=2.5pt}
\begin{table*}[t]
\centering
\vspace{6pt}
\label{table:ablation}
\begin{minipage}[t]{1\linewidth}
\centering
\renewcommand{\arraystretch}{1.1}
\begin{tabular}{>{\centering\arraybackslash}m{0.35\linewidth}>{\centering\arraybackslash}m{0.35\linewidth}>{\centering\arraybackslash}m{0.35\linewidth}>{\centering\arraybackslash}m{0.4\linewidth}}
\toprule
\multicolumn{2}{c}{Action decoder}          & \multirow{2}{*}{Instruction} & \multirow{2}{*}{Success rate} \\
Transformer          & MLP                  &                              &                               \\ \hline
\checkmark                    & \multicolumn{1}{l}{} & \multicolumn{1}{l}{}         & 50                            \\
\checkmark                    & \multicolumn{1}{l}{} & \checkmark                            & 50                            \\
\multicolumn{1}{l}{} & \checkmark                    & \multicolumn{1}{l}{}         & 50                            \\
\multicolumn{1}{l}{} & \checkmark                    & \checkmark                            & 50  \\
\bottomrule
\end{tabular}
(a) ablation study
\end{minipage}
\hspace{3.5cm}
\begin{minipage}[t]{0.2\linewidth}
\centering
\renewcommand{\arraystretch}{1.1}
\begin{tabular}{>{\centering\arraybackslash}m{0.4\linewidth}|>{\centering\arraybackslash}m{0.4\linewidth}}
\toprule
\multirow{2}{*}{Next steps} & \multirow{2}{*}{Mean} \\
                            &                       \\ \hline
N1                          & 30                    \\
N5                          & 50                    \\
N10                         & 50                    \\
N20                         & 40       \\  \bottomrule
\end{tabular}
(b) next variation
\end{minipage}
\hspace{5pt}
\begin{minipage}[t]{0.2\linewidth}
\centering
\renewcommand{\arraystretch}{1.1}
\begin{tabular}{>{\centering\arraybackslash}m{0.4\linewidth}|>{\centering\arraybackslash}m{0.4\linewidth}}
\toprule
\multirow{2}{*}{Next steps} & \multirow{2}{*}{Mean} \\
                            &                       \\ \hline
N1                          & 30                    \\
N5                          & 50                    \\
N10                         & 50                    \\
N20                         & 40       \\  \bottomrule
\end{tabular}
(c) prev variation
\end{minipage}
\caption{ablation results}
\label{table:ablation_method}
\end{table*}

==> table/ablation_step.tex <==
\captionsetup[table]{skip=2.5pt}
\begin{table}[t]
\centering
\vspace{6pt}
\label{table:ablation}
\begin{minipage}[t]{0.4\linewidth}
\centering
\renewcommand{\arraystretch}{1.3}
\begin{tabular}{>{\centering\arraybackslash}m{0.4\linewidth}|>{\centering\arraybackslash}m{0.4\linewidth}}
\toprule
\multirow{2}{*}{Next steps} & \multirow{2}{*}{Mean} \\
                            &                       \\ \hline
N1                          & 30                    \\
N5                          & 50                    \\
N10                         & 50                    \\
N20                         & 40       \\  \bottomrule
\end{tabular}
(a) next variation
\end{minipage}
\hspace{5pt}
\begin{minipage}[t]{0.4\linewidth}
\centering
\renewcommand{\arraystretch}{1.1}
\begin{tabular}{>{\centering\arraybackslash}m{0.4\linewidth}|>{\centering\arraybackslash}m{0.4\linewidth}}
\toprule
\multirow{2}{*}{Next steps} & \multirow{2}{*}{Mean} \\
                            &                       \\ \hline
N1                          & 30                    \\
N5                          & 50                    \\
N10                         & 50                    \\
N20                         & 40       \\  \bottomrule
\end{tabular}
(b) prev variation
\end{minipage}
\caption{ablation results.}
\label{table:ablation_step}
\end{table}

==> table/nextstep.tex <==
% Please add the following required packages to your document preamble:
% \usepackage{multirow}
\begin{table}[]
\centering
\renewcommand{\arraystretch}{1.3}
\resizebox{0.9\columnwidth}{!}{
\begin{tabular}{l>{\centering\arraybackslash}p{1.5cm}>{\centering\arraybackslash}p{1.5cm}>{\centering\arraybackslash}p{1.5cm}>
{\centering\arraybackslash}p{1.5cm}}
\toprule
\multirow{2}{*}{Next steps} & \multicolumn{3}{c}{Target distance} & \multirow{2}{*}{Mean} \\
                            & 0.05       & 0.075       & 0.1      &                       \\ \hline
N1                          & 20         & 30          & 40       & 30                    \\
N5                          & 20         & 30          & 40       & 50                    \\
N10                         & \textbf{20}         & \textbf{30}          & \textbf{40}       & \textbf{50}                    \\
N20                         & 20         & 30          & 40       & 40 0      \\
\bottomrule
\end{tabular}
}
\caption{Next step ablation results. Results of action decoders fed with various numbers of next steps are presented as task success percentage by the threshold distance of success.}
\label{tab:nextstep}
\end{table}

==> table/unseen.tex <==
\begin{tabular}{c|>{\centering\arraybackslash}p{1.2cm}|>{\centering\arraybackslash}p{0.8cm}>
{\centering\arraybackslash}p{0.8cm}>
{\centering\arraybackslash}p{0.8cm}|>
{\centering\arraybackslash}p{0.8cm}>
{\centering\arraybackslash}p{0.8cm}}
\toprule
\multirow{2}{*}{Model} & \multirow{2}{*}{\begin{tabular}[c]{@{}c@{}}Seen Task\\ \& Blocks\end{tabular}} & \multicolumn{3}{c|}{Unseen Task} & \multirow{2}{*}{\begin{tabular}[c]{@{}c@{}}Unseen\\ Blocks\end{tabular}} \\
                       &                                                                                     & Task 1    & Task 2    & Task 3   &               \\ \hline
Seer-S + SAVi                & 0.0                                                                                  & 0.0       & 0.0        & 0.0       & 0.5                            \\
Seer-F + SAVi                 & 0.5                                                                                  & 0.0        & 0.0        & 0.5       & 1.0                           \\
Seer-S + VAE                & 0.5                                                                                  & 0.0        & 0.0        & 0.0       & 0.0                           \\
Seer-F + VAE                & 0.5                                                                                  & 0.5        & 0.0        & 0.5       & 0.5                         \\ \hline
Ours                   & \textbf{50.0}                                                                                  & \textbf{24.5}        & \textbf{16.0}        & \textbf{26.5}       & \textbf{38.0}                            \\
\bottomrule
\end{tabular}

==> table/worldmodel_fvd.tex <==
\captionsetup[table]{skip=2.5pt}

\begin{table}[]
\centering
\setlength{\tabcolsep}{1mm}
% \renewcommand{\arraystretch}{1.3}
\begin{tabular}{lcccc}
\toprule
Model & Training Data & Number of Data   & FVD & KVD \\ \hline
Seer  & something-something v2 + language table & 13.06k & 300 & 300 \\
Seer  & language table & 0.06k  & 300 & 300 \\
Ours  & language table & 0.6k  & 300 & 300 \\
\bottomrule
\end{tabular}
\caption{KVD results.}
\label{table:worldmodel_fvd}
\end{table}

==> table/worldmodel_speed.tex <==
% \captionsetup[table]{skip=2.5pt}
% \begin{table}[]
% \centering
% \renewcommand{\arraystretch}{1.3}
% \resizebox{0.92\columnwidth}{!}{\begin{tabular}{lccc}
% \toprule
% Model & Training Data    & FVD & KVD \\ \hline
% Seer  & +launguage table & 300 & 300 \\
% Seer  & launguage table  & 300 & 300 \\ \hline
% Ours  & launguage table  & 300 & 300 \\
% \bottomrule
% \end{tabular}}
% \caption{KVD results.}
% \end{table}

% Please add the following required packages to your document preamble:
% \usepackage{multirow}
\begin{table}[]
\centering
\renewcommand{\arraystretch}{1.3}
\resizebox{\columnwidth}{!}{
\begin{tabular}{l>{\centering\arraybackslash}p{2.5cm}>{\centering\arraybackslash}p{2.5cm}}
\toprule
\multirow{2}{*}{Model} & \multirow{2}{*}{\begin{tabular}[c]{@{}c@{}}Unit Training Time\\ (s/it)\end{tabular}} & \multirow{2}{*}{\begin{tabular}[c]{@{}c@{}}Unit Inference Time\\ (s/step)\end{tabular}} \\
                       &                                                                                  &                                                                                     \\ \hline
Ours                   & 0.30                                                                              & 0.67                                                                                \\
Seer                   & 2.31                                                                             & 5.39 \\                                                                              
\bottomrule
\end{tabular}
}
\caption{speed results}
\label{table:worldmodel_speed}
\end{table}

% \begin{table}[]
% \centering
% \renewcommand{\arraystretch}{1.3}
% \resizebox{0.92\columnwidth}{!}{
% \begin{tabular}{lcc}
% \multirow{2}{*}{Model} & \multirow{2}{*}{\begin{tabular}[c]{@{}c@{}}Training Speed\\ (s/it)\end{tabular}} & \multirow{2}{*}{\begin{tabular}[c]{@{}c@{}}Inference Speed\\ (s/step)\end{tabular}} \\
%                        &                                                                                  &                                                                                     \\
% Seer                   & 0.3                                                                              & 2.31                                                                                \\
% Ours                   & 0.67                                                                             & 5.39                                                                               
% \end{tabular}
% \caption{KVD results.}
% \label{tab:my-table}
% \end{table}
